Activity River: Visualizing Planned and Logged Personal Activities for Reflection

We present Activity River, a personal visualization tool which enables individuals to plan, log, and reflect on their self-defined activities. We are interested in supporting this type of reflective practice as prior work has shown that reflection can help people plan and manage their time effectively. Hence, we designed Activity River based on five design goals (visualize historical and contextual data, facilitate comparison of goals and achievements, engage viewers with delightful visuals, support authorship, and enable flexible planning and logging) which we distilled from the Information Visualization and Human-Computer Interaction literature. To explore our approach's strengths and limitations, we conducted a qualitative study of Activity River using a role-playing method. Through this qualitative exploration, we illustrate how our participants envisioned using our visualization to perform dynamic and continuous reflection on their activities. We observed that they were able to assess their progress towards their plans and adapt to unforeseen circumstances using our tool.

==> 11_references.tex <==
\section{REFERENCES}

\begin{enumerate}

\item Sabrina Agnihotri, Joanne Rovet, Deb Cameron, Carmen Rasmussen, Jennifer Ryan, and Michelle Keightley. 2013. SenseCam as an Everyday Memory Rehabilitation Tool for Youth with Fetal Alcohol Spectrum Disorder. Proceedings of the 4th International SenseCam  \& Pervasive Imaging Conference, ACM, 86–87. http://doi.org/10.1145/2526667.2526684
\item Wolfgang Aigner, Silvia Miksch, Wolfgang Müller, Heidrun Schumann, and Christian Tominski. 2007. Visualizing time-oriented data—A systematic view. Computers  \& Graphics 31, 3: 401–409. http://doi.org/10.1016/j.cag.2007.01.030
\item Apple iOS Health App. Retrieved September 18, 2015 from www.apple.com/ios/health/
\item Marilyn P. Arnone, Ruth V. Small, Sarah A. Chauncey, and H. Patricia McKenna. 2011. Curiosity, interest and engagement in technology-pervasive learning environments: a new research agenda. Educational Technology Research and Development 59, 2: 181–198. http://doi.org/10.1007/s11423-011-9190-9
\item Eric P.S. Baumer. 2015. Reflective Informatics: Conceptual Dimensions for Designing Technologies of Reflection. Proceedings of the 33rd Annual ACM Conference on Human Factors in Computing Systems, ACM, 585–594. http://doi.org/10.1145/2702123.2702234
\item Eric P.S. Baumer, Vera Khovanskaya, Mark Matthews, Lindsay Reynolds, Victoria Schwanda Sosik, and Geri Gay. 2014. Reviewing Reflection: On the Use of Reflection in Interactive System Design. Proceedings of the 2014 Conference on Designing Interactive Systems, ACM, 93–102. http://doi.org/10.1145/2598510.2598598
\item Susan Bluck and Linda J. Levine. 1998. Reminiscence as Autobiographical Memory: A Catalyst for Reminiscence Theory Development. Ageing  \& Society 18, 02: 185–208. http://doi.org/null
\item Fred B. Bryant, Colette M. Smart, and Scott P. King. 2005. Using the Past to Enhance the Present: Boosting Happiness through Positive Reminiscence. Journal of Happiness Studies 6, 3: 227–260. http://doi.org/10.1007/s10902-005-3889-4
\item Roger Buehler, Dale Griffin, and Michael Ross. 1994. Exploring the “planning fallacy”: Why people underestimate their task completion times. Journal of Personality and Social Psychology 67, 3: 366–381. http://doi.org/10.1037/0022-3514.67.3.366
\item Lee Byron and Martin Wattenberg. 2008. Stacked Graphs: Geometry  \& Aesthetics. IEEE Transactions on Visualization and Computer Graphics 14, 6: 1245–1252. http://doi.org/10.1109/TVCG.2008.166
\item Rafael A. Calvo and Dorian Peters. 2012. Positive Computing: Technology for a Wiser World. Interactions 19, 4: 28–31. http://doi.org/10.1145/2212877.2212886
\item Jaewon Cho, Sanghoo Park, Been Jeon, Byung-Chull Bae, and Jun-Dong Cho. 2015. People's Emotional Responses to a Plant's Emotional Expression. Proceedings of the Ninth International Conference on Tangible, Embedded, and Embodied Interaction, ACM, 545–550. http://doi.org/10.1145/2677199.2687899
\item Sunny Consolvo, David W. McDonald, Tammy Toscos, et al. 2008. Activity Sensing in the Wild: A Field Trial of UbiFit Garden. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 1797–1806. http://doi.org/10.1145/1357054.1357335
\item Martin A. Conway and Christopher W. Pleydell-Pearce. 2000. The Construction of Autobiographical Memories in the Self-Memory System. Psychological Review 107, 2: 261–288. http://doi.org/10.1037/0033-295X.107.2.261
\item Daytum. Retrieved September 18, 2015 from http://www.daytum.com/
\item Nicholas Diakopoulos, Funda Kivran-Swaine, and Mor Naaman. 2011. Playable Data: Characterizing the Design Space of Game-y Infographics. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 1717–1726. http://doi.org/10.1145/1978942.1979193
\item Daniel Epstein, An Ping, James Fogarty, and Sean A. Munson. 2015. A Lived Informatics Model of Personal Informatics. UbiComp 2015. Retrieved August 27, 2015 from https://homes.cs.washington.edu/~jfogarty/publications/ubicomp2015.pdf
\item Daniel Epstein, Felicia Cordeiro, Elizabeth Bales, James Fogarty, and Sean Munson. 2014. Taming Data Complexity in Lifelogs: Exploring Visual Cuts of Personal Informatics Data. Proceedings of the 2014 Conference on Designing Interactive Systems, ACM, 667–676. http://doi.org/10.1145/2598510.2598558
\item Chloe Fan, Jodi Forlizzi, and Anind K. Dey. 2012. A Spark of Activity: Exploring Informative Art as Visualization for Physical Activity. Proceedings of the 2012 ACM Conference on Ubiquitous Computing, ACM, 81–84. http://doi.org/10.1145/2370216.2370229
\item Paul A. Fishwick. 2008. Aesthetic Computing. MIT Press.
\item Fitbit. Retrieved from www.fitbit.com
\item Mona Haraty, Diane Tam, Shathel Haddad, Joanna McGrenere, and Charlotte Tang. 2012. Individual Differences in Personal Task Management: A Field Study in an Academic Setting. Proceedings of Graphics Interface 2012, Canadian Information Processing Society, 35–44. Retrieved September 20, 2015 from http://dl.acm.org/citation.cfm?id=2305276.2305284
\item Daniel Harrison, Paul Marshall, Nadia Berthouze, and Jon Bird. 2014. Tracking Physical Activity: Problems Related to Running Longitudinal Studies with Commercial Devices. Proceedings of the 2014 ACM International Joint Conference on Pervasive and Ubiquitous Computing: Adjunct Publication, ACM, 699–702. http://doi.org/10.1145/2638728.2641320
\item Susan Havre, Elizabeth Hetzler, and Lucy Nowell. 2000. ThemeRiver: Visualizing Theme Changes Over Time. IEEE Symposium on Information Visualization, 2000. InfoVis 2000, 115–123. http://doi.org/10.1109/INFVIS.2000.885098
\item Elise van den Hoven. 2014. A Future-proof Past: Designing for Remembering Experiences. Memory Studies 7, 3: 370–384. http://doi.org/10.1177/1750698014530625
\item Dandan Huang, Melanie Tory, Bon Adriel Aseniero, et al. 2014. Personal Visualization and Personal Visual Analytics. IEEE Transactions on Visualization and Computer Graphics Early Access Online. http://doi.org/10.1109/TVCG.2014.2359887
\item I Track My Time App. Retrieved September 18, 2015 from http://reeoo.com/i-track-my-time-app
\item Cynthia S. Jacelon and Kristal Imperio. 2005. Participant Diaries as a Source of Data in Research with Older Adults. Qualitative Health Research 15, 7: 991–997. http://doi.org/10.1177/1049732305278603
\item Jawbone. Retrieved September 18, 2015 from https://jawbone.com/
\item Vaiva Kalnikaite, Abigail Sellen, Steve Whittaker, and David Kirk. 2010. Now Let Me See Where I Was: Understanding How Lifelogs Mediate Memory. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 2045–2054. http://doi.org/10.1145/1753326.1753638
\item Amirrudin Kamsin, Ann Blandford, and Anna L. Cox. 2012. Personal Task Management: My Tools Fall apart when I'M Very Busy! CHI '12 Extended Abstracts on Human Factors in Computing Systems, ACM, 1369–1374. http://doi.org/10.1145/2212776.2212457
\item Fred Korthagen. 1993. Two modes of reflection. Teaching and Teacher Education 9, 3: 317–326. http://doi.org/10.1016/0742-051X(93)90046-J
\item Fred Korthagen and Angelo Vasalos. 2005. Levels in Reflection: Core Reflection as a Means to Enhance Professional Growth. Teachers and Teaching 11, 1: 47–71. http://doi.org/10.1080/1354060042000337093
\item Lifelogging/QuantifiedSelf. Lifestream Blog.
\item Ian Li, Anind Dey, and Jodi Forlizzi. 2010. A Stage-based Model of Personal Informatics Systems. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 557–566. http://doi.org/10.1145/1753326.1753409
\item Ian Li, Anind K. Dey, and Jodi Forlizzi. 2011. Understanding My Data, Myself: Supporting Self-reflection with Ubicomp Technologies. Proceedings of the 13th International Conference on Ubiquitous Computing, ACM, 405–414. http://doi.org/10.1145/2030112.2030166
\item Ian Li, Yevgeniy Medynskiy, Jon Froehlich, and Jakob Larsen. 2012. Personal informatics in practice: improving quality of life through data. CHI '12 Extended Abstracts on Human Factors in Computing Systems, ACM, 2799–2802. http://doi.org/10.1145/2212776.2212724
\item James J. Lin, Lena Mamykina, Silvia Lindtner, Gregory Delajoux, and Henry B. Strub. 2006. Fish'n'Steps: Encouraging Physical Activity with an Interactive Computer Game. In UbiComp 2006: Ubiquitous Computing, Paul Dourish and Adrian Friday (eds.). Springer Berlin Heidelberg, 261--278. Retrieved September 18, 2015 from http://link.springer.com/chapter/10.1007/11853565\_16
\item Tom Lovett, Eamonn O'Neill, James Irwin, and David Pollington. 2010. The Calendar as a Sensor: Analysis and Improvement Using Data Fusion with Social Networks and Location. Proceedings of the 12th ACM International Conference on Ubiquitous Computing, ACM, 3–12. http://doi.org/10.1145/1864349.1864352
\item Dan P. McAdams. 1993. The Stories We Live by: Personal Myths and the Making of the Self. Guilford Press.
\item Mint. Retrieved September 18, 2015 from www.mint.com
\item Jennifer A. Moon. 2005. Reflection in Learning and Professional Development: Theory and Practice. Routledge. 
\item MyFitnessPal. Retrieved September 18, 2015 from https://myfitnesspal.com/
\item David H. Nguyen, Gabriela Marcu, Gillian R. Hayes, et al. 2009. Encountering SenseCam: Personal Recording Technologies in Everyday Life. Proceedings of the 11th International Conference on Ubiquitous Computing, \item Nike+. Retrieved September 18, 2015 from www.nikeplus.com
\item Optimized. Retrieved September 18, 2015 from http://optimized-app.com/
\item Stephen J. Payne. 1993. Understanding Calendar Use. Human-Computer Interaction. 8, 2: 83–100. http://doi.org/10.1207/s15327051hci0802\_1
\item Zachary Pousman, John T. Stasko, and Michael Mateas. 2007. Casual Information Visualization: Depictions of Data in Everyday Life. IEEE Transactions on Visualization and Computer Graphics 13, 6: 1145–1152. http://doi.org/10.1109/TVCG.2007.70541
\item QuantifiedSelf. Retrieved September 18, 2015 from http://quantifiedself.com/
\item Ioannis Refanidis and Neil Yorke-Smith. 2010. A Constraint-based Approach to Scheduling an Individual's Activities. ACM Transactions on Intelligent Systems Technology. 1, 2: 12:1–12:32. http://doi.org/10.1145/1869397.1869401
\item RescueTime. Retrieved September 18, 2015 from www.rescuetime.com
\item Johnny Rodgers and Lyn Bartram. 2011. Exploring Ambient and Artistic Visualization for Residential Energy Use Feedback. IEEE Transactions on Visualization and Computer Graphics 17, 12: 2489–2497. http://doi.org/10.1109/TVCG.2011.196
\item John Rooksby, Mattias Rost, Alistair Morrison, and Matthew Chalmers Chalmers. 2014. Personal Tracking as Lived Informatics. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 1163–1172. http://doi.org/10.1145/2556288.2557039
\item Corina Sas, Scott Challioner, Christopher Clarke, et al. 2015. Self-Defining Memory Cues: Creative Expression and Emotional Meaning. Proceedings of the 33rd Annual ACM Conference Extended Abstracts on Human Factors in Computing Systems, ACM, 2013–2018. http://doi.org/10.1145/2702613.2732842
\item Abigail J. Sellen, Andrew Fogg, Mike Aitken, Steve Hodges, Carsten Rother, and Ken Wood. 2007. Do Life-logging Technologies Support Memory for the Past?: An Experimental Study Using Sensecam. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 81–90. http://doi.org/10.1145/1240624.1240636
\item Barbara J. Speck and Stephen W. Looney. 2001. Effects of a Minimal Intervention to Increase Physical Activity. Nursing Research 50, 6: 374–378.
\item Anna Ståhl, Kristina Höök, Martin Svensson, Alex S. Taylor, and Marco Combetto. 2008. Experiencing the Affective Diary. Personal and Ubiquitous Computing 13, 5: 365–378. http://doi.org/10.1007/s00779-008-0202-7
\item Elizabeth Thiry, Siân Lindley, Richard Banks, and Tim Regan. 2013. Authoring Personal Histories: Exploring the Timeline as a Framework for Meaning Making. Proceedings of the SIGCHI Conference on Human Factors in Computing Systems, ACM, 1619–1628. http://doi.org/10.1145/2470654.2466215
\item Alice Thudt, Dominikus Baur, Samuel Huron, Sheelagh Carpendale. 2015. Visual Mementos: Reflecting Memories with Personal Data. IEEE Transactions on Visualization and Computer Graphics PP, 99: 1–1. http://doi.org/10.1109/TVCG.2015.2467831
\item Toggl. Retrieved September 18, 2015 from https://toggl.com/
\item Endel Tulving and Donald M. Thomson. 1973. Encoding Specificity and Retrieval Processes in Episodic Memory. Psychological Review 80, 5: 352–373. http://doi.org/10.1037/h0020071
\item Katerina Vrotsou, Kajsa Ellegard, and Matthew Cooper. 2007. Everyday Life Discoveries: Mining and Visualizing Activity Patterns in Social Science Diary Data. Information Visualization, 2007. IV '07. 11th International Conference, 130–138. http://doi.org/10.1109/IV.2007.48

\end{enumerate}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

